Data-CUBE: Data Curriculum for Instruction-based Sentence Representation Learning

Recently, multi-task instruction tuning has been applied into sentence representation learning, which endows the capability of generating specific representations with the guidance of task instruction, exhibiting strong generalization ability on new tasks. However, these methods mostly neglect the potential interference problems across different tasks and instances, which may affect the training and convergence of the model. To address it, we propose a data curriculum method, namely Data-CUBE, that arranges the orders of all the multi-task data for training, to minimize the interference risks from the two views. In the task level, we aim to find the optimal task order to minimize the total cross-task interference risk, which is exactly the traveling salesman problem, hence we utilize a simulated annealing algorithm to find its solution. In the instance level, we measure the difficulty of all instances per task, then divide them into the easy-to-difficult mini-batches for training. Experiments on MTEB sentence representation evaluation tasks show that our approach can boost the performance of state-of-the-art methods. Our code and data are publicly available at the link: \url{https://github.com/RUCAIBox/Data-CUBE}.

==> sec-app.tex <==
\appendix

\section*{Appendix}
% We provide some experiment-related information as supplementary materials. The appendix is organized into three sections:
% \begin{itemize}
% 	\item Statistics of each dataset are presented in Appendix~\ref{app-dataset};
% 	\item Training settings of baselines and our model PTG are presented in Appendix~\ref{app-configuration}.
% \end{itemize}



% \section{Statistics of Datasets} \label{app-dataset}
% The detailed information of the dataset for each task is listed in Table~\ref{tab:dataset}, including summarization (CNN/Daily Mail, XSum, MSNews, Multi-News and NEWSROOM), question generation (SQuAD), style transfer (Wiki Neutrality), text paraphrase (Quora), dialog (PersonaChat, TopicalChat, DailyDialog, DSTC7-AVSD and MultiWOZ) and story generation (WritingPrompts). These datasets are utilized under MIT license.

% \section{Configuration of Models} \label{app-configuration}
% %For our model, we adopt frozen BART-\textsc{large} to learn a set of source prompts. The length of prompt is set to $200$ and the learning rate is set to $1 \times 10^{-3}$. For the target generation task, we utilize BART-\textsc{large} as the generation backbone and frozen BERT-\textsc{large} to obtain the instance-level query $\bm{q}^{ins}$. The dimension $d$ is set to $1024$, which is the same as the embedding size $e$ of the BERT/BART-\textsc{large}. The multi-head attention in adaptive attention mechanism has $16$ heads. During fine-tuning, the learning rate of BART is set to $3 \times 10^{-5}$ and the learning rate of cluster key $\bm{k}^{c}$, prompt key $\bm{k}^{p}$, task key $\bm{q}^{task}$ and multi-head attention is set to $1 \times 10^{-3}$. The value of $\lambda$ is set to 0.5 based on the performance in validation set.

% The learning rate of other baselines is set to $3 \times 10^{-5}$, which is the same as our backbone BART. The other settings of baselines and our model are set the same for fair comparison. And we do not utilize special tricks such as label smoothing, warm-up learning rate and length penalty. We apply the Adam optimizer and set $\beta_1=0.9$, $\beta_2=0.98$, $\epsilon=1 \times 10^{-6}$. We set the accumulated batch size of each model to $96$ using accumulated gradients. Furthermore, we use the model with the best performance on validation set for generation. During inference, we apply the beam search method with a beam size of $5$ and a no repeat ngram size of $3$. We train our models using NVIDIA A100 GPUs and PyTorch 1.9.0 upon Ubuntu 20.04.2 LTS.


% \begin{table*}[h]
% 	\centering
% 	\begin{tabular}{lrrrrr}
% 		\toprule
% 		Dataset & \multicolumn{1}{c}{\#Train} & \multicolumn{1}{c}{\#Valid} & \multicolumn{1}{c}{\#Test} & \multicolumn{1}{c}{\#Input} & \multicolumn{1}{c}{\#Output} \\ \midrule
% 		CNN/Daily Mail & 287113 & 13368 & 11490 & 790.2 & 58.4 \\
% 		Xsum & 204017 & 11327 & 11333 & 358.8 & 21.1 \\
% 		MSNews & 136082 & 7496 & 7562 & 311.6 & 24.8 \\
% 		Multi-News & 44972 & 5622 & 5622 & 2291.9 & 263.1 \\
% 		NEWSROOM & 995040 & 108837 & 108862 & 658.5 & 26.7 \\
% 		SQuAD & 75722 & 10570 & 11877 & 148.3 & 11.6 \\
% 		Wiki Neutrality & 145197 & 18149 & 18150 & 29.1 & 27.3 \\
% 		Quora & 119410 & 14927 & 14926 & 9.8 & 9.9 \\
% 		PersonaChat & 122499 & 14602 & 14056 & 122.1 & 11.9 \\
% 		TopicalChat & 179750 & 11142 & 11221 & 216.6 & 20.3 \\
% 		DailyDialog & 76052 & 7069 & 6740 & 68.4 & 13.9 \\
% 		DSTC7-AVSD & 145521 & 33953 & 11780 & 90.7 & 9.5 \\
% 		MultiWOZ & 105115 & 13748 & 13744 & 110.7 & 13.2 \\
% 		WritingPrompts & 67765 & 3952 & 3784 & 25.7 & 232.3 \\ \bottomrule
% 	\end{tabular}
% 	\caption{Statistics of our datasets after preprocessing. \#Train, \#Valid and \#Test denote the number of examples in training, valid and test datasets, respectively. \#Input and \#Output denote the average number of tokens in the input text and output text.}
% 	\label{tab:dataset}
% \end{table*}
	



==> sec-ethic.tex <==
\section{Ethical Concerns}

% Text generation techniques has been applied to a wide range of meaningful applications for society, such as
% game narrative generation, news report generation, and weather report generation. However, this technique may be potentially utilized for harmful applications. Our work improves the quality of generated text compared with traditional methods. Thus, the high-quality text generated by our work makes it difficult to distinguish synthetic text from human-written text, such as fake news and stories. Here we are primarily concerned with two potential ethical issues: the possibility of deliberate misuse of our methodology and the issue of bias.

% First, it is somewhat challenging to anticipate the harmful usages of our method since they often involve repurposing our model in a totally different setting or for an unexpected purpose than we planned. To alleviate this issue, we can ask for the assistance of classic security risk assessment frameworks such as detecting threats. Second, biases in training data may cause our model to generate stereotyped or prejudiced texts. This is a worry since the model bias has the potential to hurt some persons in relevant groups in unforeseen ways. To avoid prejudice, it may be useful to develop a common vocabulary that connects the normative, technological, and empirical difficulties of bias reduction for our model.
